Hadamard Langevin dynamics for sampling the l1-prior

Priors with non-smooth log-densities, such as the l1-prior, are widely used in Bayesian inverse problems for their sparsity-inducing properties. Existing Langevin-based sampling methods typically rely on proximal mappings or smooth approximations, which alter the target distribution. We propose an alternative approach based on a Hadamard product parameterization of the l1-norm, leading to a smooth but nonconvex and non-globally Lipschitz potential whose marginal law exactly recovers the desired posterior. The resulting Hadamard Langevin dynamics (HLD) defines a diffusion process that is analytically distinct from proximal or mirror-type Langevin schemes. Our main contribution is a rigorous well-posedness theory for both the continuous and discrete HLD. We establish existence and uniqueness of strong solutions, geometric ergodicity of the continuous dynamics, and convergence of the discretized scheme as the step size tends to zero. These results provide the first theoretical foundation for sampling from nonconvex, nonsmooth posteriors through overparameterized Langevin dynamics.

==> macro.tex <==
\RequirePackage{mathtools,amsfonts,ifdraft,stmaryrd,microtype}
\DeclarePairedDelimiter{\Vpair}{\|}{\|} % norm like
\DeclarePairedDelimiter{\vpair}{|}{|} % abs like
\DeclarePairedDelimiter{\bpair}{[}{]} % square brackets []
\DeclarePairedDelimiter{\ppair}{(}{)} % parenthesis or round  ( )
\DeclarePairedDelimiter{\Bpair}{\{}{\}} % braces or curly { }
\DeclarePairedDelimiter{\jump}{\llbracket}{\rrbracket} % braces or curly { }
\DeclarePairedDelimiter{\ip}{\langle}{\rangle}% inner product < >
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor} % floor
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil} % ceil
%
\newcommand\strutb{\vphantom{\bigm|}}
%
\newcommand\norm[2][0pt]{\Vpair*{#2}} % ||
\newcommand\snorm[1]{\norm{\smash{#1}}} % ||
\newcommand\threenorm[1]{\lvert\!\lvert\!\lvert{#1}\rvert\!\rvert\!\rvert}
\newcommand\tvnorm[2][0pt]{\Vpair*{#2}_{\mathrm{TV}}} % ||
\newcommand\abs[2][0pt]{\vpair*{#2}} % |
\newcommand\pp[2][0pt]{\ppair*{#2}} % (
\newcommand\bp[2][0pt]{\bpair*{#2}} % [
\newcommand\Bp[2][0pt]{\Bpair*{#2}} % {
%
\newcommand\BETA{{\zeta}}
%
\newcommand\smean{\mathbb{E}}
\newcommand\mean[1]{\smean\bp{#1}}
%
\newcommand\prob{\mathbb{P}}
%
\newcommand\order[1]{\mathcal{O}\pp{#1}}
%
\newcommand\real{\mathbb{R}}

\DeclareMathOperator*{\argmin}{arg\, min}

\newcommand{\tstep}{{\Delta t}}

\renewcommand{\vec}[1]{{\mathbf{#1}}} 
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\todolist}[1]{\textcolor{red}{(TODO: #1)}}
\newcommand{\eqdef}{\coloneq}
\newcommand{\Prox}{\mathrm{Prox}}

\newcommand{\pa}[1]{\pp{#1}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\RR}{\mathbb{R}}

\newcommand{\clip}{L}
\newcommand{\clower}{K}
\newcommand{\cinfty}{B}
\newcommand{\ccc}{\clower}

\newcommand{\deltat}{{\Delta t}}
\newcommand{\deltaw}{{\Delta W}}
\newcommand{\enscond}[2]{\left\{#1:\; #2\right\}}
\newcommand{\dotp}[2]{\left<#1, #2\right>}
\newcommand{\ens}[1]{\left\{#1\right\}}



